ConTrOn: Continuously Trained Ontology based on Technical Data Sheets and Wikidata

In engineering projects involving various parts from global suppliers, one common task is to determine which parts are best suited for the project requirements. Information about specific parts' characteristics is published in so called data sheets. However, these data sheets are oftentimes only published in textual form, e.g., as a PDF. Hence, they have to be transformed into a machine-interpretable format. This transformation process still requires a lot of manual intervention and is prone to errors. Automated approaches make use of ontologies to capture the given domain and thus improve automated information extraction from the data sheets. However, ontologies rely solely on experiences and perspectives of their creators at the time of creation and cannot accumulate knowledge over time on their own. This paper presents ConTrOn -- Continuously Trained Ontology -- a system that automatically augments ontologies. ConTrOn tackles terminology problems by combining the knowledge extracted from data sheets with an ontology created by domain experts and external knowledge bases such as WordNet and Wikidata. To demonstrate how the enriched ontology can improve the information extraction process, we selected data sheets from spacecraft development as a use case. The evaluation results show that the amount of information extracted from data sheets based on ontologies is significantly increased after the ontology enrichment.

==> sections/Evaluation-IE.tex <==
\subsection{Domain Knowledge Extractor}

The purpose of this extractor is to create a group of words that represent the data sheets (topics). 
These topics will be used as context in the ontology enhancer to select a concept from external knowledge base.

The texts extracted from 170 data sheets, consists of 208 thousands words, and processed as described in Subsection \ref{sub:ie}.
We select top one thousand words to represent the data sheets.
Furthermore, we selected only the words that are defined in an English lexicon, Wordnet, so that we can analyze their meaning and context of usage.

Depends on the context, a term can be defined in different way. 
Thus, we compared all definitions of each term with the domain representatives (selected 1,000 words) and selected the definition that yields the best similarity. The excerpt of domain representatives, top ten words, are displayed in Table \ref{tab:ldasynset}

\input{tables/LDASynset.tex}

Not all selected synsets are correctly identified. 
For example, \emph{Space} and \emph{Range} are detected as verbs and provide a different meaning of the terms. 
Meanwhile, the term \emph{High} should be defined as an adjective rather than a noun in this context. 
However, as the number of data sheets increases, we will have more data to analyze and the accuracy of concept selection will be improved as well. 
A further analysis in syntax, that is to identify the function of terms before choosing their definitions, can be implemented in the future work.

